Introspective Learning : A Two-Stage Approach for Inference in Neural Networks

In this paper, we advocate for two stages in a neural network's decision making process. The first is the existing feed-forward inference framework where patterns in given data are sensed and associated with previously learned patterns. The second stage is a slower reflection stage where we ask the network to reflect on its feed-forward decision by considering and evaluating all available choices. Together, we term the two stages as introspective learning. We use gradients of trained neural networks as a measurement of this reflection. A simple three-layered Multi Layer Perceptron is used as the second stage that predicts based on all extracted gradient features. We perceptually visualize the post-hoc explanations from both stages to provide a visual grounding to introspection. For the application of recognition, we show that an introspective network is 4% more robust and 42% less prone to calibration errors when generalizing to noisy data. We also illustrate the value of introspective networks in downstream tasks that require generalizability and calibration including active learning, out-of-distribution detection, and uncertainty estimation. Finally, we ground the proposed machine introspection to human introspection for the application of image quality assessment.

==> Sections/7_Applications.tex <==
\vspace{-3mm}
\section{Applications}
\label{sec:Applications}
\vspace{-3mm}
In this section, we illustrate the advantages of introspective networks in two applications that are a function of both generalization and calibration - active learning and out-of-distribution detection. In both these applications, we show that the existing state-of-the-art methods perform better in their respective tasks and metrics if they were applied on $\mathcal{H}(\cdot)$ than on $f(\cdot)$. We then conclude by grounding the proposed introspection in neural nets with introspection in humans through IQA.
\vspace{-3mm}
\input{Tables/AL}
%\input{Tables/OOD}
\paragraph{Active Learning}
\label{subsec:AL}
The goal in active learning is to decrease the test error in a model by choosing the \textit{best} samples from a large pool of unlabeled data to annotate and train the model. A number of strategies are proposed to query the \textit{best} samples. A full review of active learning and query strategies are given in~\citet{settles2009active}. Existing active learning strategies define \textit{best} samples to annotate as those samples that the model is most uncertain about. We use the strategies given in Section~\ref{sec:Lit_review} to showcase the effectiveness of $\mathcal{H}(\cdot)$. We show the results of ResNet-18 and 34 architecture in Table~\ref{tab:AL}. Implementations of all query strategies in Table~\ref{tab:AL} are taken from the codebase of~\citet{ash2019deep} and reported as feed-forward results. Note that the query strategies act on $f(\cdot)$ to sample images at every round. In the introspective results, all query strategies sample using $\mathcal{H}(\cdot)$. The training and testing procedures strategies are the same as feed-forward from~\cite{ash2019deep}. Doing so we find similar results as recognition - on the original testset the active learning results are the same while there is a gain across strategies on Gaussian noise testset from CIFAR-10C. Note that the results shown are averaged over 20 rounds with a query batch size of a 1000 and initial random choice - which were kept same for $f(\cdot)$ and $\mathcal{H}(\cdot)$ - of 100. Further details and plots are shown in Appendix~\ref{App:AL}.
\vspace{-3mm}
\paragraph{Out-of-distribution Detection}
\label{subsec:OOD}
The goal of Out-Of-Distribution (OOD) detection is to detect those samples that are drawn from a distribution $\mathcal{X'} \neq \mathcal{X}$ given a fully trained $f(\cdot)$. As mentioned in Section~\ref{sec:Lit_review}, we use MSP~\cite{hendrycks2016baseline} and ODIN~\cite{liang2017enhancing} to illustrate the effectiveness of existing OOD methods when applied on $\mathcal{H}(\cdot)$ than if they were applied on the feed-forward $f(\cdot)$. The code for OOD detection techniques are taken from~\citet{chen2020robust} along with all hyperparameters and the training regimen. The temperature scaling coefficient for ODIN is set to $1000$. Note that we do not use additional temperature scaling on $\mathcal{H}(\cdot)$ to illustrate the effectiveness of our method. We use three established metrics to evaluate OOD detection - False Positive Rate (FPR) at 95\% True Positive Rate (TPR), Detection error, and AUROC. Ideally, AUROC values for a given method is high while the other two metrics are low. We use CIFAR-10 as our in-distribution dataset and use four OOD datasets - iSUN~\cite{xiao2010sun}, Describable Textures Dataset~\cite{cimpoi14describing}, Places 365~\cite{zhou2017places}, and LSUN~\cite{yu2015lsun}. As in recognition and active learning, we consider two difficulty settings. The first is the vanilla case with the above-listed out-of-distribution datasets. The results are presented in Appendix~\ref{App:OOD} and Table~\ref{tab:OOD_Attack}. The harder setting is when the datasets are all attacked with adversarial noise on top of being OOD. This setting is formalized in~\citet{chen2020robust}. We show these results in Table~\ref{tab:OOD}. In all cases in Table~\ref{tab:OOD}, introspection outperforms its feed-forward counterpart. In the vanilla setting, introspection is better than its feed-forward network in $15$ of considered $24$ metrics. This is inline with results from recognition and active learning where introspection generalizes better on $\mathcal{X}'$ compared to $\mathcal{X}$ testsets.



